Pre-Distribution of Entanglements in Quantum Networks

Quantum network communication is challenging, as the No-Cloning theorem in quantum regime makes many classical techniques inapplicable. For long-distance communication, the only viable approach is teleportation of quantum states, which requires a prior distribution of entangled pairs (EPs) of qubits. Establishment of EPs across remote nodes can incur significant latency due to the low probability of success of the underlying physical processes. To reduce EP generation latency, prior works have looked at selection of efficient entanglement-routing paths and simultaneous use of multiple such paths for EP generation. In this paper, we propose and investigate a complementary technique to reduce EP generation latency--to pre-distribute EPs over certain (pre-determined) pairs of network nodes; these pre-distributed EPs can then be used to generate EPs for the requested pairs, when needed, with lower generation latency. For such an pre-distribution approach to be most effective, we need to address an optimization problem of selection of node-pairs where the EPs should be pre-distributed to minimize the generation latency of expected EP requests, under a given cost constraint. In this paper, we appropriately formulate the above optimization problem and design two efficient algorithms, one of which is a greedy approach based on an approximation algorithm for a special case. Via extensive evaluations over the NetSquid simulator, we demonstrate the effectiveness of our approach and developed techniques; we show that our developed algorithms outperform a naive approach by up to an order of magnitude.

==> eaten.tex <==

\eat{
We start with describing our network protocol
to generate \epss via swapping trees.



%%%%%%%


\para{Swapping Tree Protocol.}
Our algorithms compute swapping tree(s), both SLs and non-SLs, and we need a way to implement
them on a network. 
%%%%%%%%%%
%Recent work~\cite{conext20} designed a protocol to 
%implement a {\em path}, and hence not applicable to our context.
%%%%%%%%%%%%%%%%%%%%%%%%
We build our protocol on top of the link-layer of~\cite{sigcomm19},
which is delegated with the task of continuously (when they are asked) generating \epss on a link at a desired rate (as per the swapping tree specifications).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Note that a link $(a,b)$ may be in multiple swapping trees, and hence, may need to handle multiple link-layer requests at the same time; we implement such link-layer requests by creating independent atom-photon generators at $a$ and $b$, with one pair of synchronized generators for each link-layer request. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As the links generate continuous \epss at desired rates, we need a protocol to
swap the \epss. Omitting the tedious bookkeeping details, the key aspect of the protocol
is that swap operation is done only when both the appropriate \eps pairs have arrived.
%note that the arrivals of \epss is stochastic
%in nature due to the probabilistic success swap operations at the descendants.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We implement all the gate operations (including, atomic and optical BSMs) within 
NetSquid to take the stochastic nature of quantum networks into account. 
%%%%%%%%%%%%%%%%%%%%%%
On BSM success, the swapping node transmits classical bits to the end node which manipulates its qubit, and send the final ack to the other end node. 
%%%%%%%%%%%%%%%%%%%%%%
On BSM failure, a classical ack is send to all descendant link leaves, so that they can now start accepting new link \epss; note that in our protocol, a link $l$ does not 
accept any more \epss, while its ancestor is waiting for its sibling's \eps.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The simulation has two parts. First, the network tries to generate $1/\bp^2$ amount of \epss for all the SLs' swapping  trees. The network sends and ACK to all the appropriate link-layer protocols to start producing \epss across the desired links. Different swapping (if an SL's has more than two links) will be happening to generate \epss across both SLs' ends. Left end of an SL sends an ACK to all the links involved in an SL to stop generating \epss when the sufficient amount of \epss is produced for that SL.
Second, when an (s,d) request arrives, is the way of merging different swapping trees together. Upon the arrival of the request, the network, first, sends an ACK to all the link-layer protocols assigned to that $(s,d)$ path(s) to start generating \epss across all the links. It, then, tries to do the swapping to construct both left and/or right swapping trees linked to an SL. Finally and upon constructing these swapping trees, the network will ask the proper SL to provide an \eps to do the last two swapping operations, based on the order the algorithms define.
Two cases may happen. An ACK will be sent indicating successful $(s,d)$ \eps generation if both SL's swapping are successful. After replenishing the consumed \epss for that SL, all the link-layer protocols will be turned into halt state.
If any of SL's swapping fails, the network tries to reconstruct left and/or right SL's swapping trees to continue the operations.
Note that, in both above cases, an \eps will be discarded from the SL.
}
